A Mixture-of-Expert Approach to RL-based Dialogue Management

Despite recent advancements in language models (LMs), their application to dialogue management (DM) problems and ability to carry on rich conversations remain a challenge. We use reinforcement learning (RL) to develop a dialogue agent that avoids being short-sighted (outputting generic utterances) and maximizes overall user satisfaction. Most existing RL approaches to DM train the agent at the word-level, and thus, have to deal with a combinatorially complex action space even for a medium-size vocabulary. As a result, they struggle to produce a successful and engaging dialogue even if they are warm-started with a pre-trained LM. To address this issue, we develop a RL-based DM using a novel mixture of expert language model (MoE-LM) that consists of (i) a LM capable of learning diverse semantics for conversation histories, (ii) a number of {\em specialized} LMs (or experts) capable of generating utterances corresponding to a particular attribute or personality, and (iii) a RL-based DM that performs dialogue planning with the utterances generated by the experts. Our MoE approach provides greater flexibility to generate sensible utterances with different intents and allows RL to focus on conversational-level DM. We compare it with SOTA baselines on open-domain dialogues and demonstrate its effectiveness both in terms of the diversity and sensibility of the generated utterances and the overall DM performance.

==> algorithm.tex <==
%!TEX root = main.tex

We now develop the MoE $\lambda$-PO algorithm, for which the general pseudo-code is given in Algorithm \ref{alg:train}. Recall
% from CPI analysis
that if the mixture weight $\lambda^*$ is the solution of $\arg\max_{\lambda\in\Lambda} \, \mathcal L_{f[\lambda]}$
then the MoE policy $\pi_{\lambda^*}(a|s)=\sum_{i=1}^{m-1} \lambda^*_i(s,a)\mu_i(a|s) + (1 - \sum_{i=1}^{m-1} \lambda^*_i(s,a))\mu_m(a|s)$  performs no worse than the base policy $\mu_m$. Suppose we repeat the above arguments with $\mu_j$ for each $j\in\{1,\ldots,m-1\}$, we can also show that 
\begin{small}
\begin{equation}\label{eq:gen_bdd}
    J_\pi \!-\! J_{\mu_j} \!\ge\! \frac{1}{1-\gamma}\left( L^{\prime}_{f_j[\lambda]} \!-\! \frac{\gamma}{1-\gamma}\!\cdot\! L^{\prime\prime}_{f_j[\lambda]}\!\cdot \!L^{\prime\prime\prime\prime}_{f_j[\lambda]}
    \right)\!,
\end{equation}
\end{small}
where for each $j\in\{1,\ldots,m\}$
\begin{small}
\[
f_j[\lambda]=\!\left\{\!
\begin{array}{cl}
(\lambda_1,\ldots,\lambda_{m-1},0)&\text{if $j=m$}\\
(\lambda_1, \ldots,\lambda_{j-1},0,\lambda_{j+1},\ldots, 1-\sum_{i=1}^{m-1}\lambda_i)&\text{otherwise}
\end{array}
\right.
\]
\end{small}
is a linear transformation of the mixture weight decision variable $\lambda$. To show that  $f_j[\lambda]$ is also a decision variable  $\forall j$, $j\neq m$, with respect to the corresponding base policy $\mu_j$, notice that under this transformation, whenever $\lambda$ belongs to $\Lambda$, the following conditions hold: $f_j[\lambda]\in[0,1]^{m}$, $\sum_{i=1}^{m} f_j[\lambda]_i \leq 1$, and $\sum_a\sum_{i=1}^{m}f_j[\lambda]_i(s,a)(\mu_j(a|s)-\mu_i(a|s))=0$. This means that as long as $\lambda$ belongs to feasible set $\Lambda$ the transformed mixture weight $f_j[\lambda]$ also belongs to the same feasible set $\Lambda$. Now for each $j$ we define
\begin{small}
\[
\mathcal L_{f_j[\lambda]}:=L^{\prime}_{f_j[\lambda]} \!-\! \frac{\gamma}{1-\gamma}\!\cdot\! L^{\prime\prime}_{f_j[\lambda]}\!\cdot \!L^{\prime\prime\prime\prime}_{f_j[\lambda]}.
\]
\end{small}
Then with any auxiliary convex combination weight vector $\alpha=(\alpha_1,\ldots,\alpha_m)$, i.e., $\alpha_i\geq 0$ and $\sum_{i=1}^m\alpha_i=1$, the results in \eqref{eq:bdd} and \eqref{eq:gen_bdd} imply that or any $\lambda\in\Lambda$,
\begin{small}
\begin{equation}
J_{\pi_\lambda} \geq\sum_{j=1}^m \alpha_j\left( J_{\mu_j}+\frac{\mathcal L_{f_j[\lambda]}}{1-\gamma}\right).
\end{equation}
\end{small}

\paragraph{The tabular case.}
For any arbitrary convex combination weights $\alpha$, consider the lower bound optimization problem
\begin{small}
\begin{equation}\label{problem:moe_surrogate}
\arg\max_{\lambda\in\Lambda}\sum_{j=1}^m \!\alpha_j\!\left(\! J_{\mu_j}\!+\!\frac{\mathcal L_{f_j[\lambda]}}{1-\gamma}\!\right)\!=\!\arg\max_{\lambda\in\Lambda}\sum_{j=1}^m \!\alpha_j\cdot\mathcal L_{f_j[\lambda]}.
\end{equation}
\end{small}
Recall that $\mathcal L_{f_j[\lambda]}$ is a quadratic function of $\lambda$. Therefore this optimization can be reformulated as a concave quadratic program (QP) with linear equality constraints, which has a unique optimal solution \cite{faybusovich1997infinite}. However, since the decision variable (i.e., the mixture weights) is infinite-dimensional, solving this QP is intractable without some assumptions about this mapping,  
   To resolve this issue, instead of optimizing the objective function $\sum_{j=1}^m \!\alpha_j\mathcal L_{f_j[\lambda]}$, we turn to its sample-based estimate.
   Specifically, given a batch of data \begin{small}$B_j=\{(s^{(k)},a^{(k)},\mathcal A^{(k)},r^{(k)},s^{\prime,(k)})\}_{k=1}^{|B_j|}$\end{small} generated by the behavior policy $\mu_j$, for each $j\in\{1,\ldots,m\}$, where $\mathcal A^{(k)}=\mathcal A(s^{(k)})$ is the set of candidate actions w.r.t. state $s^{(k)}$,
   we denote by \begin{small}$\lambda^{(k)}=\lambda(s^{(k)}, \cdot)\in[0,1]^{(m-1)\times |\mathcal A^{(k)}|}$\end{small} the $(m-1)\times|\mathcal A^{(k)}|$-dimensional decision variable of the mixture weight w.r.t. $k$-th data sample in $B_j$ and
   \begin{small}
   \[
   \begin{split}
   &\overline{L}^{\prime}_{f_j[\lambda]}:=\frac{1}{1-\gamma}\frac{1}{|B_j|}\sum_{i=1}^{m}\sum_{k=1}^{|B_j|}\langle f_j[\lambda^{(k)}]_i, (\mu^{(k)}_i-\mu^{(k)}_j)
    \cdot A^{(k)}_{\mu_j}\rangle_k\\
   &\overline{L}^{\prime\prime}_{f_j[\lambda]}:=\frac{1}{1-\gamma}\frac{1}{|B_j|}\sum_{i=1}^{m}\sum_{k=1}^{|B_j|}\langle f_j[\lambda^{(k)}]_i,|\mu^{(k)}_i-\mu^{(k)}_j|\rangle_k\\
   &\overline{L}^{\prime\prime\prime\prime}_{f_j[\lambda]}:=\frac{1}{1-\gamma}\frac{1}{|B_j|}\sum_{i=1}^{m}\sum_{k=1}^{|B_j|}\langle f_j[\lambda^{(k)}]_i, |(\mu^{(k)}_i-\mu^{(k)}_j)
    \cdot A^{(k)}_{\mu_j}|\rangle_k
   \end{split}
   \]
   \end{small}
   the sample-average approximation (SAA) of functions ${L}^{\prime}_{f_j[\lambda]}$, ${L}^{\prime\prime}_{f_j[\lambda]}$, and ${L}^{\prime\prime\prime\prime}_{f_j[\lambda]}$ respectively, where \begin{small}$f_j[\lambda^{(k)}]=f_j[\lambda(s^{(k)}, \cdot)]\in [0,1]^{m\times|\mathcal A^{(k)}|}$\end{small}, \begin{small}$|\mu^{(k)}_i-\mu^{(k)}_j|=\{|\mu_i(a|s^{(k)})-\mu_j(a|s^{(k)})|\}_{a\in\mathcal A^{(k)}}\in\mathbb R^{|\mathcal A^{(k)}|}$\end{small}, and  \begin{small}$(\mu^{(k)}_i-\mu^{(k)}_j)\cdot A^{(k)}_{\mu_j}=\{(\mu^{(k)}_i(a|s^{(k)})-\mu^{(k)}_j(a|s^{(k)})) \cdot A^{(k)}_{\mu_j}(s^{(k)},a)\}_{a\in\mathcal A^{(k)}}\in\mathbb R^{|\mathcal A^{(k)}|}$\end{small} such that each element generated by a sample from $B_j$, and $\langle x^{(k)},y^{(k)}\rangle_k=\sum_{a\in\mathcal A^{(k)}}x^{(k)}(a)\cdot y^{(k)}(a)$ is an inner product over the set of candidate actions $\mathcal A^{(k)}$.
   Since the expectation in ${L}^{\prime}_{f_j[\lambda]}$, ${L}^{\prime\prime}_{f_j[\lambda]}$, and  \begin{small}${L}^{\prime\prime\prime\prime}_{f_j[\lambda]}$\end{small} is over the stationary distribution induced by the base policy $\mu_j$, all SAA functions are \emph{unbiased} Monte-Carlo estimates of their population-based counterparts. We now define \begin{small}$\overline{\mathcal L}_{f_j[\lambda]}:=\overline{L}^{\prime}_{f_j[\lambda]}- \overline{L}^{\prime\prime}_{f_j[\lambda]}\cdot\overline{L}^{\prime\prime\prime\prime}_{f_j[\lambda]}$\end{small} as the $j$-th SAA objective function and consider the SAA-maximization problem
   \begin{small}\begin{equation}
   \begin{split}
  &\arg\max_{\lambda\in\overline \Lambda}\sum_{j=1}^m\!\!\Bigg(\!\sum_{i=1}^{m}\!\langle f_j[\overline\lambda]_i, (\mu_i\!-\!\mu_j)
    \cdot \alpha_j A_{\mu_j}\rangle\!-\!\frac{\gamma}{|B|(1-\gamma)}\cdot\\
    &\,\sum_{i=1}^{m}\langle f_j[\overline\lambda]_i,|\mu_i-\mu_j|\rangle\cdot\sum_{i=1}^{m}\langle f_j[\overline\lambda]_i, |(\mu_i\!-\!\mu_j)
    \cdot \alpha_j A_{\mu_j}|\rangle\!\Bigg),
    \end{split}
\end{equation}
\end{small}
where the above inner products $\langle\cdot,\cdot\rangle$ sums over both data samples and corresponding candidate actions at each batch $B_j$, $\forall j$, and the feasible set \begin{small} $\overline\Lambda=\{\overline\lambda\in[0,1]^{|\bigcup_{j=1}^m B_j|\cdot |\bigcup_{j=1}^m\mathcal A(B_j)|\cdot(m-1)}:\sum_{i=1}^{m-1}\overline\lambda[s,a,i]\leq 1,\forall a\in\mathcal A^{(k)},\,\sum_{a\in \mathcal A^{(k)}}\sum_{i=1}^{m-1}\overline\lambda[s,a,i]\cdot (\mu_i(a|s)-\mu_m(a|s))=0,\forall s\in\bigcup_{j=1}^m B_j\}$\end{small} only imposes constraints on the states that appear in the data.

This finite-dimensional linear constrained QP problem can be expressed in the following quadratic form:
\begin{small}
\[
\max_{\lambda\in\overline \Lambda}\,\,\sum_{j=1}^m \lambda^\top D[f]^\top_j \left( (\mathcal U\!-\!\mu_j)
    \cdot \alpha_j A_{\mu_j}\right)
-\frac{1}{2}\cdot \lambda^\top (D[f]^\top_j \Theta_j D[f]_j ) \lambda,
\]
\end{small}
where \begin{small}$D[f] =\{\nabla_{\lambda} f_j[\lambda^{(k)}]_{i}\}_{k\leq |B_j|, j\leq m, i\leq m}$\end{small}, is a \begin{small}$|\bigcup_{j=1}^m B_j|\cdot |\bigcup_{j=1}^m\mathcal A(B_j)|\cdot m\times |\bigcup_{j=1}^m B_j|\cdot |\bigcup_{j=1}^m\mathcal A(B_j)|\cdot(m-1)$\end{small} matrix that is independent of $\lambda$ because for each $j\in\{1,\ldots,m\}$, $f_j[\cdot]$ is a linear transformation function of $\lambda$, \begin{small}$(\mathcal U\!-\!\mu_j)
    \cdot \alpha_j A_{\mu_j}=\{(\mu^{(k)}_i-\mu^{(k)}_j)\cdot\alpha_j A^{(k)}_{\mu_j}\}_{k\leq |B_j|,j\leq m, i\leq m}$\end{small} is a $|\bigcup_{j=1}^m B_j|\cdot |\bigcup_{j=1}^m\mathcal A(B_j)|\cdot m$ dimensional vector, the series of symmetric quadratic matrices in the QP is given by
\begin{small}
\[
\Theta_{j}:=\frac{\gamma (D_{|\alpha_j A_{\mu_j}|}\cdot \Delta_{\mathcal U,\mu_j}+ \Delta_{\mathcal U,\mu_j}\cdot D_{|\alpha_j A_{\mu_j}|}^\top)}{|B_j|(1-\gamma)},\forall j,
\]
\end{small}
\begin{small}
$\Delta_{\mathcal U,\mu_j}=|\mathcal U\!-\!\mu_j|\cdot|\mathcal U\!-\!\mu_j|^\top$\end{small}, and 
\begin{small}$D_{| \alpha_j A_{\mu_j} |}=\text{diag}(\{|\alpha_j A^{(k)}_{\mu_j} |\}_{k\leq |B_j|,j\leq m})\otimes I_{m}$\end{small} is a \begin{small}$|\bigcup_{j=1}^m B_j|\cdot |\bigcup_{j=1}^m\mathcal A(B_j)|\cdot m\times |\bigcup_{j=1}^m B_j|\cdot |\bigcup_{j=1}^m\mathcal A(B_j)|\cdot m$\end{small}-diagonal matrix whose elements are the absolute advantage function. Here the transpose operation $x^\top y$ sums over (i) all mixture weights, (ii) data samples, and (iii) the corresponding candidate actions at each batch $B_j$, $\forall j$. By definition, $\Theta$ is positive-semi-definite, hence the QP above is concave. 

Using its KKT condition, the unique optimal mixture weight vector is given as
\begin{small}
\begin{align}
&\overline\lambda^*\! =\!\max\!\big(0,(\sum_{j}\!D[f]_j^\top\Theta_j D[f]_j)^{-1}( \sum_j D[f]_j \cdot (\mathcal U\!-\!\mu_j)
    \cdot \alpha_j A_{\mu_j}\nonumber\\
& \quad\quad + M_{\mu}^\top\nu_{\mu}- N^\top\max\{0,\kappa\})\big),
   \label{eq:lambda_vector}
\end{align}
\end{small}
where 
\begin{small}
\[
M_{\mu}=\text{blkdiag}(\{[(\mu^{(k)}_1-\mu^{(k)}_m),\ldots, (\mu^{(k)}_{m-1}-\mu^{(k)}_m)]\}_{k\leq |B_j|,j\leq m})
\]
\end{small}
is a $|\bigcup_{j=1}^m B_j|\times|\bigcup_{j=1}^m B_j|\cdot |\bigcup_{j=1}^m\mathcal A(B_j)|\cdot (m-1)$-matrix, 
\begin{small}
$N=\mathbf 1_{m-1}\footnote{$\mathbf 1_d$ is a $d$-dimensional vector of all 1's.}\otimes I_{k\leq |B_j|,j\leq m}$
\end{small}
is a $|\bigcup_{j=1}^m B_j|\cdot |\bigcup_{j=1}^m\mathcal A(B_j)|\times|\bigcup_{j=1}^m B_j|\cdot |\bigcup_{j=1}^m\mathcal A(B_j)|\cdot (m-1)$-matrix, $\nu_{\mu}\in\mathbb{R}^{|\bigcup_{j=1}^m B_j|}$ is the Lagrange multiplier w.r.t. constraint $M_{\mu}\overline \lambda=0$ and $\max\{\kappa,0\}$, such that $\kappa\in\mathbb{R}^{|\bigcup_{j=1}^m B_j|\cdot|\bigcup_{j=1}^m\mathcal A(B_j)|}$, is the Lagrange multiplier w.r.t. constraint $N\overline\lambda\leq 1$. Invoking the KKT conditions, the Lagrange multipliers can be found by solving the following equations:
\begin{small}
\begin{align}
\nu_{\mu}&=-H_\mu^{-1} M_{\mu}(\sum_{j}D[f]_j^\top\Theta_j D[f]_j)^{-1}\cdot(L_\mu-N^\top\max\{0,\kappa\}),\nonumber\\
\kappa&=K^{-1} \big(N(\sum_{j}D[f]_j^\top\Theta_j D[f]_j)^{-1}\cdot(L_\mu+M_\mu^\top\nu_\mu)-e\big),\nonumber
\end{align}
\end{small}
where $H_\mu=M_{\mu}(\sum_{j}D[f]_j^\top\Theta_j D[f]_j)^{-1}M_{\mu}^\top$, $K=N(\sum_{j}D[f]_j^\top\Theta_j D[f]_j)^{-1}N^\top$, $L_\mu=\sum_j D[f]_j \cdot (\mathcal U\!-\!\mu_j)
    \cdot \alpha_j A_{\mu_j}$, and $e=\mathbf 1_{|\bigcup_{j=1}^m B_j|\cdot |\bigcup_{j=1}^m\mathcal A(B_j)|}$.
    
With the optimal SAA mixture weight vector $\overline\lambda^*$ computed using the dataset $\bigcup_{j=1}^m B_j$, we then construct the mixture weight function $\lambda(s,a)$ in the 
following tabular fashion:
$$
\lambda(s,a)=\left\{\begin{array}{cl}
   \overline\lambda^*_{s,a}  &  \text{if $(s,a)\in \bigcup_{j=1}^m B_j$}\\
    0 & \text{otherwise}
\end{array}\right. .
$$
While this construction preserves optimality w.r.t.\ the surrogate MoE RL problem in (\ref{problem:moe_surrogate}), it may be overly conservative, because the policy equates to the base policy $\mu_m$ by setting $\lambda=\mathbf 0$ at state-action pairs that are not in $\bigcup_{j=1}^m B_j$. To alleviate this conservative-ness, we propose to learn a mixture weights that generalize to out-of-distribution samples.
%This sets the confidence at all state-action pairs that do not belong to $B$ to zero. While this construction generally has no loss of optimality w.r.t.\ the CPI objective (\ref{problem:crpo})---the samples have measure zero w.r.t.\ data distribution $\visitbehavior$---constructing a residual policy with this confidence function may be overly conservative, because this policy equates to the behavior policy at state-action pairs that are not in $B$ (i.e., no policy improvement). To alleviate this conservatism, we propose the following methods to learn a confidence function that generalizes to out-of-distribution samples.

\paragraph{Function Approximation.}
Given a confidence vector $\overline\lambda^*$ corresponding to samples in batch $B_1\cup B_2,\ldots\cup B_m$ and the corresponding mixture weight distribution samples $\rho_{\overline\lambda^*}$, we learn the general mixture weight distribution $\rho_\phi(s,a):\Sset\times\Aset \rightarrow [0,1]^{m}$ in a supervised fashion. 

To ensure that this function satisfies the constraint: $\lambda_\phi(s,a)\in\Lambda(s,a)$, i.e., $\sum_a\sum_{i=1}^{m-1}\lambda_{\phi,i}(s,a)(\mu_i(a|s)-\mu(a|s))=0$, $\lambda_{\phi,}(s,a)\in[0,1]$, $\forall s,a$\footnote{If one restricts $\lambda_\phi$ to be only \emph{state}-dependent,  this constraint immediately holds.}, we parameterize it as
\begin{small}
\begin{equation}
\lambda_{\phi^*}(s,a):=\frac{\pi_{\phi^*}(a|s)-\mu(a|s)}{\rho(a|s)-\mu(a|s)},\,\,\forall (s,a)\in S\times A,
\end{equation}
\end{small}
where $\pi_\phi\in\Delta$ is a learnable policy mapping, such that $\min\{\mu(a|s),\rho(a|s)\}\leq\pi_\phi(a|s)\leq\max\{\mu(a|s),\rho(a|s)\}$, $\forall s,a$. We then learn $\phi$ via the following KL distribution-fitting objective
\cite{rusu2015policy}:
\begin{small}
\[
\min_{\phi}\frac{1}{B}\sum_{(s,a)\in B}\!\!\pi_\phi(a|s)\log\left(\frac{\pi_\phi(a|s)}{(1-\overline\lambda^*_{s,a})\mu(a|s)+\overline\lambda^*_{s,a}\cdot\rho(a|s)}\right).
\]
\end{small}
While this approach learns 
% a confidence function 
$\lambda_\phi$ by generalizing the confidence vector to out-of-distribution samples, when $\pi_\phi$ is a NN, one challenge is to 
% implicitly 
enforce the constraint: $\min\{\mu(a|s),\rho(a|s)\}\leq\pi_\phi(a|s)\leq\max\{\mu(a|s),\rho(a|s)\}$, $\forall s,a$. Instead, 
% inspired by OptNet \cite{amos2017optnet}, 
using an in-graph convex optimization NN \cite{amos2017optnet}, we parameterize $\lambda_\phi$ with a NN with the following \emph{constraint-projection layer} $\Phi:S\rightarrow A$ before the output:
\begin{align}
\Phi(s)\in&\arg\min_{\lambda\in \mathbb{R}^{|A|}}\,\frac{1}{2}\sum_{a\in A}\|\lambda_a-\widetilde\lambda^*_{s,a}\|^2,\nonumber\\
\text{s.t.}&\, \sum_a\lambda_a(\rho(a|s)-\mu(a|s))=0,\,\,0\leq \lambda\leq 1,\label{eq:optimize_lambda}
\end{align}
where, at any $s\in S$, the $|A|$-dimensional confidence vector label $\{\widetilde\lambda^*_{s,a}\}_{a\in A}$ is equal to 
% the vector 
$\{\overline\lambda^*_{\overline{s},a}\}_{a\in A}$ chosen from the batch confidence vector $\overline\lambda^*$ such that $\overline{s}$ in $B$ is closest to $s$. Indeed, analogous to the closed-form solution 
% of the confidence vector 
in (\ref{eq:lambda_vector}), this projection layer has a closed-form QP formulation
with linear constraints:
$
\Phi(s)=\min\{1,\max\{0,\widetilde\lambda^*_{s,\cdot}+(\rho(\cdot|s)-\beta(\cdot|s))\cdot\mu_{\beta,\rho}\}\}
$,
where Lagrange multiplier $\mu_{\beta,\rho}$ is given by
$
\mu_{\mu,\rho}\!=\!-{(\rho(\cdot|s)-\beta(\cdot|s))^\top\widetilde\lambda^*_{s,\cdot}}/{\|\rho(\cdot|s)-\beta(\cdot|s)\|^2}.
$


\begin{algorithm}[th!]
\caption{MoE RL algorithm}\label{alg:train}
\begin{algorithmic}[1]
\Require{ $B$: batch data; Tunable parameter $\mu\in[0,1]$ }
\For{$t=1,\ldots,N$}
    \State Sample mini-batch of transitions $(s, a, r, d, s')\sim B$
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % lambda update
    \State Compute $\overline\lambda^*$ from Eq.~(\ref{eq:lambda_vector})
    \State Update confidence $\phi^*$ by Eq.~(\ref{eq:optimize_lambda})
        \State Update candidate policy $\rho^*_{\lambda_{\phi^*}}$ by Eq.~(\ref{eq:relateive_soft})
    % Q-update
    \State Construct target critic network $V_{\theta'}(s') \!:=$\\
    $\qquad\ (1-\mu)\mathbb{E}_{a'\sim\beta}[Q_{\theta'}(s',a')] + \mu \max_{a'} Q_{\theta'}(s',a')$
    
    %\Comment{See section~\ref{sec:bcrpo} for the analysis in the case $\mu=1$}
    \State Update $\theta \leftarrow \argmax_{\theta}\frac{1}{2}\left(
        Q_{\theta}(s,a) - r - \gamma V_{\theta'}(s')\right)^2$
    \State Update target network: $\theta'\leftarrow \tau \theta + (1-\tau)\theta'$
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\EndFor
\end{algorithmic}
\end{algorithm}

% The confidence can be represented by a separate neural network jointly trained with the $Q$-function. One possible simplification is to make it depends only on state, but not action. In that way, the constraint is reduced to $\mix[(s)] \in [0, 1]$, which can be easily implemented using a sigmoid function. In addition to the supervised learning approach using the closed-form QP solution as label, one can update the network by taking gradient step that maximizes Equation~\ref{problem:crpo_mu_2}, treating $\rho$ as constant.



==> practical_implementation.tex <==
%!TEX root = main.tex
In this section, we discuss several practical techniques to further boost training stability and effectiveness of \BCRPO{}.

\paragraph{Improving CPI with Optimal Advantage}
The derivation in Section \ref{sec:bcrpo} and Section \ref{sec:algorithm} shows that optimizing  $\mathcal{L}_{\pibehavior,\rho,\lambda}$ finds a residual policy that performs no-worse than the behavior policy (modulo any Lagrangian approximation error).
While we argue that this optimization is less conservative than existing methods (like TRPO) due to the state-action-dependent learned confidence, it might not be aggressive enough in leveraging the function approximation to generalize to unseen state and action.
% Although we argue that this optimization would be less conservative compared to TRPO (due to the state-action-dependent learned confidence), in practice this CPI objective function can still be too conservative; i.e., the solution policy $\pi$ will end up being very close to $\pibehavior$.
One major reason is that by design, $\mathcal{L}_{\pibehavior,\rho,\lambda}$ only uses the long-term value of $\pibehavior$ (in the form of $A_\pibehavior$), in order to circumvent the issue of bad generalization to unseen state-action pair. This also makes policy improvement local to $\pibehavior$. This is a fundamental challenge of batch RL, but can be relaxed depending on the domain.
% (in both the radius of the policy trust region around $\pibehavior$  and the linear objective function).
As a remedy to this issue, by a convex ensemble of the results from Lemma \ref{lem:main} and Theorem \ref{thm:main} (with any combination weight $\mu\in[0,1]$), notice that the difference-return also satisfies
\[
J_\pi - J_\beta \ge \frac{1}{1-\gamma} \left( \widetilde{L}^{\prime}_{\mu,\pibehavior,\rho,\lambda} - \frac{\gamma(1-\mu)}{1-\gamma} L^{\prime\prime}_{\pibehavior,\rho,\lambda}\max_{s_0\in S}\, L^{\prime\prime\prime}_{\pibehavior,\rho,\lambda}(s_0)
    \right),
\]
where 
\[
\widetilde{L}^{\prime}_{\mu,\pibehavior,\rho,\lambda}:= \E_{(s,a)\sim \visitbehavior}\left[
    \mix \cdot\frac{\rho(a|s)-\pibehavior(a|s)}{\pibehavior(a|s)} \cdot
    W(s,a)
    \right]
    \]
    with a \emph{weighted advantage} function $W:= (1-\mu) \adv[\pibehavior] + \mu \adv[\pi]$.
Therefore, without loss of generality one can replace $A_\pibehavior$ in
% $L^{\prime}_{\pibehavior,\rho,\lambda}$ of
$\mathcal{L}_{\pibehavior,\rho,\lambda}$ with the weighted advantage function. Furthermore, to avoid estimating $A_\pi$ at each policy update and assuming that CPI eventually finds $\pi\rightarrow\pi^*$, one may directly estimate the optimal weighted advantage function 
$$W_{\pi^*}(s,a)= Q_{\mu,\beta,\pi^*}(s,a)-V_{\mu,\beta,\pi^*}(s),$$ in which the value function $Q_{\mu,\beta,\pi^*}$ is a Bellman fixed-point of  $Q(s,a)=R(s,a)+\gamma\sum_{s'}T(s'|s,a) V(s')$, with
\[
V(s) = (1-\mu)\mathbb E_{a\sim\pibehavior}[Q(s,a)]+\mu \max_{a}Q(s,a).
\]
This approach of combining the optimal Bellman operator with the on-policy counterpart belongs to the general class of hybrid on/off-policy RL algorithms~\cite{o2016combining}. 


Therefore,
% in order to reduce the conservative-ness of BRPO,
we learn an advantage function $W$ that is a weighted combination of $A_\pibehavior$ and $A_{\pi^*}$.
Using the batch data $B$, the expected advantage $A_\pibehavior$ can be learned with any critic-learning technique, such as SARSA~\cite{sutton2018reinforcement}.
We can learn $A_{\pi^*}$ by DQN~\cite{mnih2013playing} or other Q-learning algorithm.
We provide pseudo-code of our \BCRPO{} algorithm in Algorithm~\ref{alg:train}.

==> proofs_cm.tex <==
%!TEX root = main.tex

We begin by defining and characterizing the \emph{difference-value function},
a concept we exploit in the derivation of our MoE RL algorithms. For notational convenience, we first focus on the difference-value derivation with respect to base policy $\Psi_p$ and the remaining base policies $\{\Psi_j\}_{i=1}^{p-1}$. Similar results can be extended to any arbitrary base policies.
For any state-action pair $(s,a)\in \Sset\times\Aset$, let $V_{\pi_\Lambda}(s)$ and $V_{\Psi_p}(s)$ ($Q_{\pi_\Lambda}(s,a)$ and $Q_{\Psi_p}(s,a)$) be the (state-action) value functions induced by policies $\pi_\Lambda$ and ${\Psi_p}$, respectively. 
Using the structure of the residual policy,  we establish two characterizations of the \emph{difference-value function} $\Delta Q_{\pi_\Lambda,{\Psi_p}}(s):=Q_{\pi_\Lambda}(s,a)-Q_{\Psi_p}(s,a)$.
% that corresponds to ${\Psi_p}$ and $\pi_\Lambda$.
\begin{lemma}\label{lem:main}
Let $A_{\pi_\Lambda}(s,a):=Q_{\pi_\Lambda}(s,a)-V_{\pi_\Lambda}(s)$ be the advantage function w.r.t. MoE policy $\pi_\Lambda$.
The difference-value is
\begin{small}
\[
\Delta Q_{\pi_\Lambda,{\Psi_p}}(s,a)\!=\!\mathbb E_{P,{\Psi_p}} [ \sum_{t=0}^\infty\gamma^t\Delta\widehat{A}_{\pi,\Lambda}(s_t,a_t)\!\mid\! s_0=s, a_0=a ],
\]
\end{small}
where with $f[\Lambda]=(\Lambda_1,\ldots,\Lambda_{p-1},0)$
\begin{small}
$\Delta\widehat{A}_{\Lambda}(s,a) = \left( \sum_{j=1}^{p}f[\Lambda]_j\cdot\frac{\Psi_j - {\Psi_p}}{{\Psi_p}}\cdot \adv[\pi]\right)(s, a)$
\end{small}
is the difference reward that depends on mixture weight $\Lambda$. 
\end{lemma}
\begin{proof}
% Before going into the derivation of this theorem, we first have the following technical result that studies the distance of the occupation measures that are induced by $\Psi_p$ and $\pi_\Lambda$.

Consider the following chain of equalities from matrix manipulations:
\begin{small}
\[
\begin{split}
&(I-\gamma P_{\Psi_p})^{-1}\cdot(I-\gamma P_{\pi_\Lambda})\\
=&(I-\gamma P_{\Psi_p})^{-1}\cdot\left(I-\gamma  \left\{\sum_{a\in A} P(s'|s,a)\left(\Psi_p(a|s)+ \sum_{j=1}^{p-1}\Lambda_j(s,a) (\Psi_j(a|s)-\Psi_p(a|s))\right)\right\}_{s,s'}\right)\\
=&\left(I-\gamma(I-\gamma P_{\Psi_p})^{-1}\left\{ \sum_{a\in A} P(s'|s,a)\sum_{j=1}^{p-1}\Lambda_j(s,a) (\Psi_j(a|s)-\Psi_p(a|s))\right\}_{s,s'\in S}\right).
\end{split}
\]
\end{small}
By multiplying the matrix $(I-\gamma P_{\pi_\Lambda})^{-1}$ on both sides of the above expression, it implies that
\begin{small}
\[
\begin{split}
(I-\gamma P_{\Psi_p})^{-1}-(I-\gamma P_{\pi_\Lambda})^{-1}=&-\left(\gamma(I-\gamma P_{\Psi_p})^{-1}\left\{ \sum_{a\in A} P(s'|s,a)\sum_{j=1}^{p-1}\Lambda_j(s,a)(\Psi_j(a|s)-\Psi_p(a|s))\right\}_{s,s'\in S}(I-\gamma P_{\pi_\Lambda})^{-1}\right).
\end{split}
\]
\end{small}
This implies that
\begin{small}
\[
\left((I-\gamma P_{\pi_\Lambda})^{-1} -(I-\gamma P_{\Psi_p})^{-1}\right)(s'|s)=-\gamma(I-\gamma P_{\Psi_p})^{-1}\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda}(I-\gamma P_{\pi_\Lambda})^{-1}(s'|s),
\]
\end{small}
where $P_{\pi_\Lambda}(s'|s)$ and $P_{\Psi_p}(s'|s)$ represent the transition probabilities from state $s$ to next-state $s'$ following policy $\pi_\Lambda$ and $\Psi_p$ respectively, and for any state-next-state pair $(s,s')$, 
\begin{small}
\[
\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda}(s'|s)=\sum_{a\in A} P(s'|s,a)\Psi_p(a|s)\cdot \sum_{j=1}^{p-1}\Lambda_j(s,a) \cdot\frac{\Psi_j(a|s)-\Psi_p(a|s)}{\Psi_p(a|s)}.
\]
\end{small}

Using the above result, for any initial state $s\in S$, the value functions that are induced by $\Psi_p$ and $\pi_\Lambda$ have the following relationship:
\begin{small}
\begin{equation}\label{eq:intermediate}
\begin{split}
V_{\pi_\Lambda}(s)-V_{\Psi_p}(s)=&\delta_{s_0=s}^\top(I-\gamma P_{\pi_\Lambda})^{-1} R_{\pi_\Lambda}-\delta_{s_0=s}^\top(I-\gamma P_{\Psi_p})^{-1} R_{\Psi_p}\\
=&\delta_{s_0=s}^\top\left((I-\gamma P_{\pi_\Lambda})^{-1} -(I-\gamma P_{\Psi_p})^{-1}\right) R_{\pi_\Lambda} + \delta_{s_0=s}^\top(I-\gamma P_{\Psi_p})^{-1}\left( R_{\pi_\Lambda}- R_{\Psi_p}\right)\\
= &\gamma\cdot\mathbb E_{P,\Psi_p}\left[\sum_{t=0}^\infty\gamma^t\sum_{j=1}^{p-1}\Lambda_j(s_t, a_t)\cdot \frac{\Psi_j(a_t|s_t)-\Psi_p(a_t|s_t)}{\Psi_p(a_t|s_t)}\cdot V_{\pi_\Lambda}(s_{t+1})\mid s_0=s\right] \\
&\quad+\mathbb E_{P,\Psi_p}\left[\sum_{t=0}^\infty\gamma^t \sum_{j=1}^{p-1}\Lambda_j(s_t, a_t) \cdot \frac{\Psi_j(a_t|s_t)-\Psi_p(a_t|s_t)}{\Psi_p(a_t|s_t)}\cdot R(s_t,a_t)\mid s_0=s\right]\\
= & \mathbb E_{P,\Psi_p}\left[\sum_{t=0}^\infty\gamma^t \sum_{j=1}^{p-1}\Lambda_j(s_t, a_t) \cdot \frac{\Psi_j(a_t|s_t)-\Psi_p(a_t|s_t)}{\Psi_p(a_t|s_t)}\cdot Q_{\pi_\Lambda}(s_t,a_t)\mid s_0=s\right]\\
=&\mathbb E_{P,\Psi_p}\left[\sum_{t=0}^\infty\gamma^t \sum_{j=1}^{p-1}\Lambda_j(s_t, a_t) \cdot \frac{\Psi_j(a_t|s_t)-\Psi_p(a_t|s_t)}{\Psi_p(a_t|s_t)}\cdot A_{\pi_\Lambda}(s_t,a_t)\mid s_0=s\right].
\end{split}
\end{equation}
\end{small}
The second equality follows from the fact that 
$
Q_{\pi_\Lambda}(s,a) = R(s,a) + \gamma\sum_{s'\in S}P(s'|s,a)V_{\pi_\Lambda}(s').
$
The third equality follows from the above result  and the fact that for any state $s\in S$, $(I-\gamma P_{\pi_\Lambda})^{-1}R_{\pi_\Lambda}(s)=V_{\pi_\Lambda}(s)$. The last equality is based on the fact of the confidence constraint that 
\begin{small}
\[
\mathbb E_{P,\Psi_p}\left[\sum_{t=0}^\infty \gamma^t V_{\pi_\Lambda}(s_t)\cdot\sum_{a}\sum_{j=1}^{p-1}\Lambda_j(s_t, a)\cdot(\Psi_j(a|s_t)- \Psi_p(a|s_t))\mid s_0=s\right] = 0,\,\,\forall s\in S.
\]
\end{small}
\end{proof}

This result establishes that the difference value is essentially a value function w.r.t.\ a specific difference reward. 
 While the difference value can be estimated from behavior data batch,  this formulation requires knowledge of the advantage function $A_{\pi_\Lambda}$ w.r.t.\ the MoE policy $\pi_\Lambda$. Alternatively, we can show that the difference value can 
also be expressed as a function of the advantage w.r.t.\
the \emph{base policy} ${\Psi_p}$:
\begin{theorem}\label{thm:main}
Let $A_{\Psi_p}(s,a)\!:=\!Q_{\Psi_p}(s,a)\!-\!V_{\Psi_p}(s)$ be the behavior advantage function. The difference-value is 
\begin{small}\[\Delta Q_{\pi_\Lambda,{\Psi_p}}(s,a)\!=\!\mathbb E_{P,\pi}\left[\sum_{t=0}^\infty\!\gamma^t\Delta A_{\Lambda}(s_t,a_t)\!\!\mid\!\! s_0=s,a_0=a\right],\]\end{small}
where with $f[\Lambda]=(\Lambda_1,\ldots,\Lambda_{p-1},0)$
\begin{small}
$
\Delta A_{\Lambda}(s,a)=\left({\Psi_p}\cdot\sum_{j=1}^{p}f[\Lambda]_j\cdot\frac{\Psi_j - {\Psi_p}}{{\Psi_p}}\cdot \adv[{\Psi_p}]\right)(s, a)
$
\end{small}
is the behavior difference reward that depends on mixture weight $\Lambda$. 
\end{theorem}
\begin{proof}
Denote by $V_{\pi_\Lambda}$ and $V_{\Psi_p}$ the vectors of value functions $V_{\pi_\Lambda}(s)$ and $V_{\Psi_p}(s)$ at every state $s\in S$ respectively. Re-writing the result in (\ref{eq:intermediate}) in matrix form, it can be expressed as
\[
V_{\pi_\Lambda}-V_{\Psi_p}=(I-\gamma P_{\Psi_p})^{-1}\left(\Delta R_{\Psi_p,\Psi_{1:p-1},\Lambda}+\gamma\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda}V_{\Psi_p}+\gamma\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda}(V_{\pi_\Lambda}-V_{\Psi_p})\right),
\]
where for any state $s\in S$, 
\[
\Delta R_{\Psi_p,\Psi_{1:p-1},\Lambda}(s)=\sum_{a}\Psi_p(a|s)\cdot \sum_{j=1}^{p-1}\Lambda_j(s,a) \cdot \frac{\Psi_j(a|s)-\Psi_p(a|s)}{\Psi_p(a|s)}\cdot R(s,a),
\] and 
\[
\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda}(s'|s)=\sum_{a\in A} P(s'|s,a)\Psi_p(a|s)\cdot \sum_{j=1}^{p-1}\Lambda_j(s,a) \cdot\frac{\Psi_j(a|s)-\Psi_p(a|s)}{\Psi_p(a|s)}.
\]
This expression implies that
\[
(I - (I-\gamma P_{\Psi_p})^{-1}\gamma\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda})(V_{\pi_\Lambda}-V_{\Psi_p})=(I-\gamma P_{\Psi_p})^{-1}(\Delta R_{\Psi_p,\Psi_{1:p-1},\Lambda}+\gamma\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda}V_{\Psi_p}),
\]
which further implies that
\[
V_{\pi_\Lambda}-V_{\Psi_p}=(I - (I-\gamma P_{\Psi_p})^{-1}\gamma\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda})^{-1}(I-\gamma P_{\Psi_p})^{-1}\left(\Delta R_{\Psi_p,\Psi_{1:p-1},\Lambda}+\gamma\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda}V_{\Psi_p}\right).
\]
Here based on the definition of $\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda}$ and the confidence constraint, one can show that $(P_{\Psi_p}+\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda})$ is a stochastic matrix (all the elements are non-negative, and $\sum_{s'\in S}(P_{\Psi_p}+\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda})(s'|s)=1$, $\forall s\in S$). Therefore the matrix $(I - (I-\gamma P_{\Psi_p})^{-1}\gamma\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda})$ is invertible. 

Using the matrix inversion lemma, one has the following equality:
\begin{small}
\[
(I - (I-\gamma P_{\Psi_p})^{-1}\cdot\gamma\cdot\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda})^{-1}=(I-\gamma (P_{\Psi_p}+\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda}))^{-1}(I-\gamma P_{\Psi_p}).
\]
\end{small}
Therefore the difference of value function $V_{\pi_\Lambda}-V_{\Psi_p}$ can further be expressed as
\begin{small}
\[
V_{\pi_\Lambda}-V_{\Psi_p}=(I-\gamma P_{\Psi_p}-\gamma\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda})^{-1}\left(\Delta R_{\Psi_p,\Psi_{1:p-1},\Lambda}+\gamma\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda}V_{\Psi_p}\right).
\]
\end{small}
In other words, at any state $s\in S$, the corresponding value function $V_{\pi_\Lambda}(s)$ is given by the following expression:
\begin{small}
\begin{equation}
\begin{split}
V_{\pi_\Lambda}(s)-V_{\Psi_p}(s)=&\mathbb E\left[\sum_{t=0}^\infty\gamma^t\left(\Delta R_{\Psi_p,\Psi_{1:p-1},\Lambda}+\gamma\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda}V_{\Psi_p}\right)(s_t)\mid P'_{\Psi_p,\Psi_{1:p-1}},s_0=s\right]\\
=&\mathbb E\left[\sum_{t=0}^\infty\gamma^t\Delta Q_{\Psi_p,\Psi_{1:p-1},\Lambda}(s_t,a_t)\mid P'_{\Psi_p,\Psi_{1:p-1}},s_0=s\right]\\
=&\mathbb E\left[\sum_{t=0}^\infty\gamma^t\Delta A_{\Psi_p,\Psi_{1:p-1},\Lambda}(s_t,a_t)\mid P'_{\Psi_p,\Psi_{1:p-1}},s_0=s\right],
\end{split}
\end{equation}
\end{small}
where the transition probability $P'_{\Psi_p,\Psi_{1:p-1}}(s'|s)=(P_{\Psi_p}+\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda})(s'|s)$ is given by $\sum_{a\in A}\Psi_p(a|s)\cdot P(s'|s,a)\cdot\left(1+ \sum_{j=1}^{p-1}\Lambda_j(s,a) \cdot\frac{\Psi_j(a|s)-\Psi_p(a|s)}{\Psi_p(a|s)}\right)$ at state-next-state pair $(s,s')$. By noticing that $P'_{\Psi_p,\Psi_{1:p-1}}(s'|s)$ is indeed $P_\pi(s'|s)$ (the transition probability that is induced by residual policy $\pi_\Lambda$), the proof of Theorem \ref{thm:main} is completed.
\end{proof}

In MoE-MDP, we exploit the
nature of the difference-value function to solve the maximization w.r.t.\ the mixture weight: $\Lambda^*(s,a)\!\in \argmax_{\Lambda\in \Lambda(s,a)}\Delta Q_{\pi_\Lambda,\Psi_p}(s,a)$, $\forall (s,a)\in \Sset\times\Aset$. 
While the above reformulation cannot change the fact that the original MoE RL problem is NP-hard, the main motivation of using the difference-value formulation is to derive an effective $\Lambda$-policy optimization algorithm, especially in the batch setting, where learning with off-policy data to well-known to incur instability due to high generalization error \citep{kumar2019stabilizing}. Specifically our approach below is based on adopting the CPI methodology \citep{kakade2002approximately} and reducing its conservative-ness by leveraging the special structure of the difference-value function.


\begin{lemma}\label{thm:cpi_2_1}
The difference return of $(\pi_\Lambda,\Psi_p)$ satisfies
\begin{small}
\begin{equation}\label{eq:bdd}
    J_{\pi_\Lambda} \!-\! J_{\Psi_p} \!\ge\! \frac{1}{1-\gamma}\left( L^{\prime}_{f[\Lambda]} \!-\! \frac{\gamma}{1-\gamma}\!\cdot\! L^{\prime\prime}_{f[\Lambda]}\!\cdot \!\max_{s_0\in S}\,L^{\prime\prime\prime}_{f[\Lambda]}(s_0)
    \right)\!,
\end{equation}
\end{small}
where with $f[\Lambda]=(\Lambda_1,\ldots,\Lambda_{p-1},0)$ the surrogate objective function, regularization, and penalty weight are
\begin{small}
\begin{equation*}
\begin{split}
    L^{\prime}_{f[\Lambda]}\!:=& \E_{d_{\Psi_p}}\!\left[
    \sum_{j=1}^{p}\!\left(f[\Lambda]_j \!\cdot\!\frac{\Psi_j-\Psi_p}{\Psi_p} \!\cdot\!
    A_{\Psi_p}\right)(s,\!a)
    \!\right]\\
    L^{\prime\prime}_{f[\Lambda]}\!:=& \E_{ d_{\Psi_p}}\!\left[\sum_{j=1}^{p}\!
    \left(f[\Lambda]_j \!\cdot\!\frac{\left|\Psi_j-\Psi_p\right|}{\Psi_p}\right)(s,\!a)\!\right]\\
    L^{\prime\prime\prime}_{f[\Lambda]}(s_0)\!:=& \E_{d_{\Psi_p}(s_0)} \left[|A_{\Psi_p}|\!\cdot\!\sum_{j=1}^{p}\!
    \left(f[\Lambda]_j\!\cdot\!\frac{\left|\Psi_j\!-\!\Psi_p\right|}{\Psi_p}\right)(s,\!a) \!\right]
\end{split}
\end{equation*}
\end{small}
respectively, in which $d_{\Psi_p}(s_0)$ is the discounted occupancy measure w.r.t. $\Psi_p$ given initial state $s_0$.
\end{lemma}
\begin{proof}
Define the state-action discounted stationary distribution w.r.t. an arbitrary policy $\pi_\Lambda$ as 
$d_{\pi_\Lambda}(s,a)=(1-\gamma)\sum_{t=0}^\infty\gamma^t \mathbb P(s_t=s,a_t=a|s_0\sim  P_0,\pi)$ and its state-only counterpart as $d_{\pi_\Lambda}(s)=\sum_{a\in A}d_{\pi_\Lambda}(s,a)\pi(a|s)$.
Immediately one can write the difference of return (objective function of this problem) with the following chain of equalities/inequalities:

\begin{small}
\begin{align*}
\E\left[\sum_{t=0}^\infty \gamma^t\Delta A_{\Psi_p,\Psi_{1:p-1},\Lambda}(s_t)\mid P, \pi, s_0 \right]
&=\frac{1}{1-\gamma}\sum_{s\in S}d_{\pi_\Lambda}(s)\Delta A_{\Psi_p,\Psi_{1:p-1},\Lambda}(s)\\
&=\frac{1}{1-\gamma}\sum_{s\in S}d_{\Psi_p}(s)\Delta A_{\Psi_p,\Psi_{1:p-1},\Lambda}(s)+ (d_{\pi_\Lambda}(s)-d_{\Psi_p}(s))\Delta A_{\Psi_p,\Psi_{1:p-1},\Lambda}(s).
\end{align*}
\end{small}

Recall that 
\begin{small}
\[
\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda}(s'|s)=\sum_{a\in A} P(s'|s,a)\Psi_p(a|s)\cdot \sum_{j=1}^{p-1}\Lambda_j(s,a) \cdot\frac{\Psi_j(a|s)-\Psi_p(a|s)}{\Psi_p(a|s)}.
\]
\end{small}
At any state $s\in S$, the difference of stationary distribution $d_{\pi_\Lambda}(s)-d_{\Psi_p}(s)$ can be further expressed as
\begin{small}
\[
\begin{split}
 (d_{\pi_\Lambda}-d_{\Psi_p}&)(s)
 = \delta_{s=s_0}^\top\left((I-\gamma P_{\pi_\Lambda})^{-1}-(I-\gamma P_{\Psi_p})^{-1}\right)(s)\\
 =& \delta_{s=s_0}^\top\big((I-\gamma P_{\Psi_p})^{-1}+(I-\gamma P_{\Psi_p})^{-1}\gamma\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda}(I-(I-\gamma P_{\Psi_p})^{-1}\gamma\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda})^{-1}\cdot\\
&\qquad\qquad(I-\gamma P_{\Psi_p})^{-1}-(I-\gamma P_{\Psi_p})^{-1}\big)(s)\\
 =& \delta_{s=s_0}^\top\left((I-\gamma P_{\Psi_p})^{-1}\gamma\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda}(I-(I-\gamma P_{\Psi_p})^{-1}\gamma\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda})^{-1}(I-\gamma P_{\Psi_p})^{-1}\right)(s).
 \end{split}
\]
\end{small}
 
Let 
\begin{small}
\[
D_{\Psi_p}=\left\{(1-\gamma)\cdot\E[\sum_{t=0}^\infty\gamma^t\mathbb P (s_t=s'|s_0=s,\Psi_p)]\right\}_{s,s'\in S}
\]
\end{small}
be the occupation measure matrix induced by $\Psi_p$. Combining the above arguments one has
\begin{small}
\begin{align}
& \left|\langle d_{\pi_\Lambda}-d_{\Psi_p},\Delta A_{\Psi_p,\Psi_{1:p-1},\Lambda}\rangle\right|\label{eq:abs_diff}\\
= &\left|\langle \delta_{s=s_0}^\top(I-\gamma P_{\Psi_p})^{-1}\gamma\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda}(I-(I-\gamma P_{\Psi_p})^{-1}\gamma\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda})^{-1}(I-\gamma P_{\Psi_p})^{-1},\Delta A_{\Psi_p,\Psi_{1:p-1},\Lambda}\rangle\right|\nonumber\\
= &\frac{1}{1-\gamma}\left|\langle \delta_{s=s_0}^\top D_{\Psi_p}\gamma\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda}((1-\gamma)I-D_{\Psi_p}\gamma\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda})^{-1},D_{\Psi_p}\Delta A_{\Psi_p,\Psi_{1:p-1},\Lambda}\rangle\right|\nonumber\\
= &\frac{\gamma}{1-\gamma}\left|\langle \delta_{s=s_0}^\top D_{\Psi_p}\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda},\left( I -\gamma \left(I+D_{\Psi_p}\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda}\right)\right)^{-1}D_{\Psi_p}\Delta A_{\Psi_p,\Psi_{1:p-1},\Lambda}\rangle\right|.\nonumber
\end{align}
\end{small}
Now $I+D_{\Psi_p}\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda}$ is a stochastic matrix, which is because for any state $s\in S$,
\begin{small}
\begin{align*}
(D_{\Psi_p}\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda}e)(s) &= (1-\gamma) \E \left[\sum_{t=0}^\infty \gamma^t\sum_{s'}\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda}(s'|s)\mid P,\beta, s_0=s \right]\\
&=(1-\gamma)\E\left[\sum_{t=0}^\infty \gamma^t\sum_{a\in A} \sum_{j=1}^{p-1}\Lambda_j(s,a) \cdot(\Psi_j(a|s)-\Psi_p(a|s))\mid P,\beta, s_0=s \right]\\
&=0.
\end{align*}
\end{small}
Using this property one can upper bound the magnitude of each element of matrix $\left( I -\gamma \left(I+D_{\Psi_p}\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda}\right)\right)^{-1}$ by $\frac{1}{1-\gamma}$. Therefore, using Holder inequality one can further upper bound the expression in (\ref{eq:abs_diff}) as follows:
% \[
% \begin{split}
% & \left|\langle d_{\pi_\Lambda}-d_{\Psi_p},\Delta A_{\Psi_p,\Psi_{1:p-1},\Lambda}\rangle\right|\leq \frac{\gamma}{(1-\gamma)^2}\left\| \delta_{s=s_0}^\top D_{\Psi_p}\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda}\right\|_1\cdot\left\|D_{\Psi_p}\Delta A_{\Psi_p,\Psi_{1:p-1},\Lambda}\right\|_\infty\\
%  \leq& \frac{\gamma}{(1-\gamma)^2}\sum_{s\in S,a\in A}d_{\Psi_p}(s)\Psi_p(a|s)\cdot \Lambda(s,a) \cdot\frac{|\Psi_j(a|s)-\Psi_p(a|s)|}{\Psi_p(a|s)}\cdot \max_{s_0\in S}\sum_{s\in S}d_{\Psi_p}(s|s_0)\left|\Delta A_{\Psi_p,\Psi_{1:p-1},\Lambda}\right|.
%  \end{split}
% \]
\begin{small}
\begin{align*}
&\left|\langle d_{\pi_\Lambda}-d_{\Psi_p},\Delta A_{\Psi_p,\Psi_{1:p-1},\Lambda}\rangle\right|
\leq \frac{\gamma}{(1-\gamma)^2}\left\| \delta_{s=s_0}^\top D_{\Psi_p}\Delta P_{\Psi_p,\Psi_{1:p-1},\Lambda}\right\|_1\cdot\left\|D_{\Psi_p}\Delta A_{\Psi_p,\Psi_{1:p-1},\Lambda}\right\|_\infty\\
&\qquad\qquad\leq \frac{\gamma}{(1-\gamma)^2}\sum_{s\in S,a\in A}d_{\Psi_p}(s)\Psi_p(a|s)\cdot \sum_{j=1}^{p-1}\Lambda_j(s,a) \cdot\frac{|\Psi_j(a|s)-\Psi_p(a|s)|}{\Psi_p(a|s)}\cdot \max_{s_0\in S}\sum_{s\in S}d_{\Psi_p}(s|s_0)\left|\Delta A_{\Psi_p,\Psi_{1:p-1},\Lambda}\right|.
 \end{align*}
 \end{small}
Plugging in the definition of the discounted occupation measure w.r.t. $\Psi_p$ into the above expression, the proof is this theorem is completed. 
\end{proof}

Notice that the lower bound in Lemma \ref{thm:cpi_2_1} is comprised only of terms that can be estimated directly
using the data batch $B$ (generated by $\Psi_p$). In practice it is reasonable to approximate $\max_{s_0\in\Sset}L^{\prime\prime\prime}_{f[\Lambda]}(s_0)$ with $\mathbb E_{s_0}[L^{\prime\prime\prime}_{f[\Lambda]}(s_0)]$. The main reason behind this claim is because when $\gamma$ is large enough (e.g., in dialogue management $\gamma$ is often greater than $0.9$), under the assumption of an irreducible Markov chain $P_{\Psi_p}$ the occupancy measure $d_{\Psi_p}$ is equal to the stationary distribution of this Markov chain and is therefore independent of initial state. 
 Theoretical results to support this hypothesis can be derived through connecting the mixing time \cite{mixing_markov} of the Markov chain $P_{\Psi_p}$ with the effective horizon of the $\gamma$-discounting MDP but is left for future work.
 
Now with \begin{small}\[
L^{\prime\prime\prime\prime}_{f[\Lambda]}:=\mathbb E_{s_0}[L^{\prime\prime\prime}_{f[\Lambda]}(s_0)]=\E_{d_{\Psi_p}} [\sum_{j=1}^{p}(
    f[\Lambda]_j\!\cdot\!\frac{|\Psi_j-\Psi_p|}{\Psi_p}\!\cdot\! |A_{\Psi_p}|)(s,a) ],
    \]\end{small}
    the terms $L_{W,f[\Lambda]}$, $L^{\prime}_{f[\Lambda]}$, $L^{\prime\prime}_{f[\Lambda]}$, and $L^{\prime\prime\prime\prime}_{f[\Lambda]}$ are all linear in $\Lambda$; thus our lower bound in \eqref{eq:bdd} is quadratic in $\Lambda$---this modification ensures the optimal $\Lambda$ solved by maximizing the lower bound is not
a \emph{degenerate extreme point} of $\mathcal{G}$.\footnote{Notice that vanilla CPI has a linear objective function in $\Lambda$ and simplex constraints. Therefore the optimal $\Lambda^*$ will always be a $0-1$ vector. When \begin{small}$\frac{2 \gamma}{1-\gamma}\E_{ d_{\Psi_p}}\left[\sum_{j=1}^{p}
    \sqrt{\frac{1}{2}
    % \kl{\Psi_p(s)}{\Psi_j(s)}
    \kl{\Psi_p(s)}{\Psi_j(s)}
    }\,\right]$\end{small} is large, then $\Lambda^*$ will be forced to minimize $\mathbb E_{\pi, P}[\Delta U]$, for which an immediate solution is $\Lambda^*=\mathbf{0}$, i.e.,  $\pi_{\Lambda^*}={\Psi_p}$.}
Although this lower bound maximziation problem can be reformulated as quadratic programming, in the realm of dialogue management when the MoE-CM $\Lambda$ is parameterized with a complex function approximation, e.g., NN, solving this problem in practice may still be computationally expensive. 

\subsection{Proof of Theorem \ref{thm:cpi_2_1}}
To make the aforementioned lower bound optimization problem more tractable, one approach is to first further lower bound \eqref{eq:bdd} with the following series of inequalities: 
\begin{small}
\[
\begin{split}
\frac{1}{1-\gamma}\left( L^{\prime}_{f[\Lambda]} \!-\! \frac{\gamma\!\cdot\! L^{\prime\prime}_{f[\Lambda]}\!\cdot \!L^{\prime\prime\prime\prime}_{f[\Lambda]}}{1-\gamma}\right)\geq & \frac{1}{1-\gamma}\E_{d_{\Psi_p}}\!\left[
    \pi_\Lambda\cdot\!
    A_{\Psi_p}(s)\right]-\frac{\gamma\|A_{\Psi_p}\|_\infty}{(1-\gamma)^2} \E_{ d_{\Psi_p}}\!\left[\|\pi_\Lambda-\Psi_p\|_1(s)\right]^2\\
\geq & \frac{1}{1-\gamma}\E_{d_{\Psi_p}}\!\left[
\pi_\Lambda\cdot\!
A_{\Psi_p}(s)\right]-\frac{\gamma\|A_{\Psi_p}\|_\infty}{(1-\gamma)^2} \E_{ d_{\Psi_p}}\!\left[\|\pi_\Lambda-\Psi_p\|_1^2(s)\right]\\
\geq & \E_{d_{\Psi_p}}\!\left[
\frac{\pi_\Lambda\cdot\!
A_{\Psi_p}(s)}{1-\gamma}-\frac{\gamma\|A_{\Psi_p}\|_\infty}{2(1-\gamma)^2}\cdot\kl{\pi_\Lambda}{\Psi_p}(s)\right], 
\end{split}
\]
\end{small}
where the first inequality is based on the definition of MoE-LM and the Holder inequality, the second inequality is based on the Cauchy-Schwartz inequality, and the third inequality is based on the Pinsker inequality. 

\subsection{A TRPO Baseline Approach}
Alternatively we have the following baseline approach, which directly extends from Corollary~1 of TRPO \citep{schulman2015trust} (for multiple candidate policies) to ensure  $\pi_\Lambda$ performs no worse than $\Psi_p$.
\begin{lemma}\label{lem:cpi_1}
For any value function $W:S\to\R$, the return of $\pi_\Lambda$ satisfies
\begin{small}
\[
J_{\pi_\Lambda} -J_{\Psi_p}  \ge \frac{1}{1-\gamma} L_{W,f[\Lambda]} - \frac{2 \gamma}{(1-\gamma)^2} \cdot \epsilon_{W} \cdot \E_{s\sim d_{\Psi_p}}\left[\sum_{j=1}^{p}
    f[\Lambda]_j\sqrt{\frac{1}{2}
    \kl{\Psi_p(\cdot|s)}{\Psi_j(\cdot|s)}
    }
    \right],
\]\end{small}
where with $f[\Lambda]=(\Lambda_1,\ldots,\Lambda_{p-1},0)$ and $\Delta W(s,a,s') := R(s,a) + \gamma W(s') - W(s)$ the surrogate objective and the penalty weight are given by
\begin{small}
\begin{equation*}
\begin{split}
&L_{W,f[\Lambda]} \!:=\! \mathbb E_{d_{\Psi_p}}\!\!\left[\!\sum_{j=1}^{p}\!
    \left(f[\Lambda]_j\!\cdot\!\frac{\Psi_j\!-\!\Psi_p}{\Psi_p}
    \right)(s,\!a)\cdot\Delta W(s,a,s')\!
    \right],\,\,\epsilon_{W} \!:=\! \max_{s} |\E_{\pi_\Lambda, P}[\Delta W(s,a,s')]|.\, 
\end{split}
\end{equation*}
\end{small}
\end{lemma}
When $W = V_{\pi_\Lambda}$, one has $\Delta W=A_{\pi_\Lambda}$, where $A_{\pi_\Lambda}=Q_{\pi_\Lambda}-V_{\pi_\Lambda}$ is the advantage function of $\pi_\Lambda$, and $\E_{\pi_\Lambda,P}[\Delta W]=0$, which implies that the inequality is tight---this lemma then
coincides Lemma~\ref{lem:main}.  Although theoretically when $\pi_\Lambda$ is optimal, $\epsilon_{W}=\mathbb E_{\pi_\Lambda,P}[A_{\pi_\Lambda}]$ should be zero, in practice the main issue of using TRPO in MoE-CM optimization is on the approximation of $\epsilon_{W}$ with $\hat\epsilon_{W}$, which replaces the advantage function $A_{\pi_\Lambda}$ with its value function estimate. With a large generalization error in off-policy value learning of $A_{\pi_\Lambda}$, it may turn out \begin{small}$O(\hat\epsilon_{W} / (1-\gamma))>>O(|L_{W,f[\Lambda}]|)$\end{small}, which results in an algorithm that is overly conservative, i.e., it only makes small improvements over base policy ${\Psi_p}$.

To compare the bounds in TRPO (Lemma \ref{lem:cpi_1}) and Theorem \ref{thm:cpi_2}, recall that the MoE-LM policy can be written as \begin{small}\[\pi_\Lambda(a|s)=\sum_{j=1}^{p-1} \Lambda_j(s,a)\Psi_j(a|s)+(1-\sum_{j=1}^{p-1} \Lambda_j(s,a))\Psi_p(a|s).\]\end{small}
With the popular value-function choice of $\Delta W=A_{\Psi_p}$, 
the term $
    L_{W,f[\Lambda]}$ in the TRPO bound
is equal to the term \begin{small}$\E_{s\sim d_{\Psi_p}}\left[
\pi_\Lambda\!\cdot\!
A_{\Psi_p}\!(s)\right]$\end{small} in Theorem \ref{thm:cpi_2}. To show that the KL-divergence term in the TRPO bound has the same magnitude with that in Theorem \ref{thm:cpi_2}, for any state $s\in S$, Pinsker's inequality \cite{pinsker} implies that \begin{small}
\[
    D_{\text{TV}}(\pi_\Lambda(\cdot|s)||\Psi_p(\cdot|s)=O(
    \sqrt{D_{\text{KL}}(\pi_\Lambda(\cdot|s)||\Psi_p(\cdot|s)}).
    \]\end{small}
    Together with the convexity of TV-divergence and Pinsker's inequality, one further has 
    \begin{small}
    \[
    D_{\text{TV}}(\pi_\Lambda(\cdot|s)||\Psi_p(\cdot|s)) \leq \sum_{j=1}^p f[\Lambda]_j
    D_{\text{TV}}(\Psi_j(\cdot|s)||\Psi_p(\cdot|s))\leq \sum_{j=1}^{p}f[\Lambda]_j
    \sqrt{\frac{1}{2}
    \kl{\Psi_p(\cdot|s)}{\Psi_j(\cdot|s)}.
    }
    \]
    \end{small} The main difference between the TRPO bound and that in Theorem \ref{thm:cpi_2} is in the remaining term, where with function approximation error the term $\hat\epsilon_{W}$ in TRPO may be much larger than $\E_{s\sim d_{\Psi_p}}[\|\!A_{\Psi_p}\!\|_\infty\sqrt{\kl{\pi_\Lambda}{\Psi_p}(s)}]$ in Theorem \ref{thm:cpi_2}, especially when the policies are close to each other.

==> related_work.tex <==
 %!TEX root = main.tex
Since our MoE LM work consists both designing specialized LMs and using RL for dialogue management, we divide this section into (i) Steerable LMs, and (ii) RL for dialogue management. 
\paragraph{Steerable LMs}{Recent work on LMs leverages deep neural networks (DNNs) to avoid hand-crafted summary states and actions \cite{gavsic2011line}. While approaches such as \citet{fatemi2016policy} and \citet{liu2018dialogue} encode conversation to a low-dimensional continuous-valued dialogue state with an RNN or transformer model, the output of these models predict a small number of dialogue acts (e.g., slot-value pairs) in task-based domains, and it is unclear how to extend these approaches to controlled text generation. Several works have considered ways \citep{ziegler2019fine, kikuchi2016controlling, ficler2017controlling} of systematically steering LMs for  conditional text generation. However, to generate texts for each specific intent or topic, the entire model needs to be separately fine-tuned, and doing so is expensive \citep{keskar2019ctrl}. In contrast, the modular structure of our hierarchical LM does not require
retraining the entire generative model. Similar to \cite{gu2017trainable, chen2018stable, subramani2019can, dathathri2019plug}, our approach designs a steerable LM that consists of a more organized representation space such that contents correspond to sampling from different regions of this space.}

\paragraph{RL for Dialogue Management}{The use of RL for dialogue management has traditionally focused on task-oriented problems, which are modeled as MDPs \citep{levin1997stochastic, singh2002optimizing, walker2000application} or POMDPs \citep{williams2007partially, young2010hidden}, 
% These problems usually have limited number of task-specific actions \citep{fatemi2016policy, gavsic2011line, su2017sample, liu2018dialogue}, which can be solved via the much simpler slot-filling approach. 
which optimizes either user feedback \citep{shah2018bootstrapping} or other explicit signals, e.g., task completion rate \citep{shi2018sentiment}. Recently RL for open-domain dialogue has also become quite popular. Examples include training a simple RL model to pick utterances generated by MLE-based dialogue models to answer a user’s query \citep{serban2017deep}, or applying deep RL to learn a word-level generative model conditioned on the dialogue history for open-domain chat \citep{jaques2019way, li2016deep, li2017adversarial, shin2020generating}. While the first approach has very limited applications, the second approach suffers from the complexity of optimizing over a very large action space, in which the word-level RL decoder may perform planning poorly, leading to incomprehensible utterances \citep{zhao2019rethinking}.
Our proposed hierarchical LM aims to achieve the best of both worlds, where candidate utterances are first generated by the lower-level LM and dialogue planning is subsequently done on a more abstract (latent) action space. Similar approaches can be found in \cite{zhao2019rethinking,saleh2020hierarchical}, which assumes problem-specific LM structures, and in MILABOT \citep{serban2017deep}, where the dialogue manager selects a response from several generated candidates. However, none of these approaches learns both the candidate generation LMs and the dialogue manager. This important difference allows our LM to compose richer responses and make decisions more effectively. 

Designing rewards for RL dialogue management has always been an active research topic. Earlier work optimizes certain hand-crafted rewards that described qualities
of the generated text, e.g., conversation length \citep{zhou2020design}, or ease of answering \citep{li2016deep}. Some approaches  train a
discriminator to distinguish human from generated text as a reward \citep{li2017adversarial, li2019dialogue} or used implicit signals such as sentiment \citep{hancock2019learning} as rewards for RL. However, these signals are usually a mix of user and bot based signals, which cannot directly optimize for user response. Our proposed MoE LM systematically utilizes bot-based rewards to first train specialized bot LMs and let RL optimize for user responses, which would arguably be more efficient.
}
